HEp-2 Cell Classification via Fusing Texture and Shape Information

Indirect Immunofluorescence (IIF) HEp-2 cell image is an effective evidence for diagnosis of autoimmune diseases. Recently computer-aided diagnosis of autoimmune diseases by IIF HEp-2 cell classification has attracted great attention. However the HEp-2 cell classification task is quite challenging due to large intra-class variation and small between-class variation. In this paper we propose an effective and efficient approach for the automatic classification of IIF HEp-2 cell image by fusing multi-resolution texture information and richer shape information. To be specific, we propose to: a) capture the multi-resolution texture information by a novel Pairwise Rotation Invariant Co-occurrence of Local Gabor Binary Pattern (PRICoLGBP) descriptor, b) depict the richer shape information by using an Improved Fisher Vector (IFV) model with RootSIFT features which are sampled from large image patches in multiple scales, and c) combine them properly. We evaluate systematically the proposed approach on the IEEE International Conference on Pattern Recognition (ICPR) 2012, IEEE International Conference on Image Processing (ICIP) 2013 and ICPR 2014 contest data sets. The experimental results for the proposed methods significantly outperform the winners of ICPR 2012 and ICIP 2013 contest, and achieve comparable performance with the winner of the newly released ICPR 2014 contest.

==> algorithm.tex <==




%\begin{multicols}{2}
\begin{figure}[t]
\begin{center}
 \includegraphics[width=1.0\linewidth]{figures/ulbp.eps}
\end{center}
   \caption{All 58 uniform LBP patterns are divided into 9 groups. In each group, any one pattern can rotate to any another pattern. The patterns in the same group has the same number of ``1'' and ``0''.}
\label{fig:ulbp}
\end{figure}
%\end{multicols}
\section{A Brief Review of LBP}
\label{sec:LBP}
LBP is an effective texture descriptor that depicts the local structures of natural images, such as edge, contour, flat region and so on. For each pixel in an image, the LBP pattern can be computed by comparing its pixel value with the values of surrounding neighbors:
%\begin{equation}
%    LBP_{P, R} = \sum_{p=0}^{P-1} s(v_p-v_c)2^p, \ \ \ \ \
%    s(x) = \begin{cases}
%    1, &  x \ge 0 \\
%    0, &  x < 0, \\
%    \end{cases}
%\end{equation}
%
%\begin{equation}
%\mathcal{P}_{c,i}(s) = \sum_{p=0}^{P-1} s(v_p-v_c)2^p, \ \ \ \ \
%s(x) = \begin{cases}
%1, & x \ge 0 \\
%0, & x < 0, \\
%\end{cases}
%\end{equation}


\begin{equation}
LBP(\vec{s}) = \sum_{k=0}^{n-1} \phi(v_k-v_c)2^k, \ \ \ \ \
\phi(x) = \begin{cases} 1, & x \ge 0 \\
0, & x < 0, \\
\end{cases}
\end{equation}
where $\vec{s} = [n, r]$, $n$ is the number of neighbors and $r$ is the radius of the neighbors. $v_c$ is the gray value of the central pixel, and $v_k$ is the value of its $k$-th neighbor.






In \cite{ojala2002multiresolution}, Ojala et al. observed that these patterns with very few spatial transitions described the fundamental properties of the image, and they called these patterns as ``uniform patterns''. The number of spatial transitions can be calculated as follows:
\begin{equation}
    \Phi(LBP(\vec{s})) = \sum_{k=1}^{n} |\phi(v_k-v_c) - \phi(v_{k-1}-v_c)|,
\end{equation}
where $v_n$ equals to $v_0$. The uniform patterns are defined as these patterns with $\Phi(LBP(s)) \le 2$. For instance, LBP patterns ``00000000'' and ``00001110'' are the uniform patterns, while ``00100100'' and ``01001110'' are non-uniform patterns.

The uniform LBP ($LBP^{U}$) depends on the start point of the binary sequence. Defined on different start points, $LBP^{U}$ will have different uniform patterns. For instance, the binary sequence ``00001000'' defined on 1$st$ position or 2$nd$ position, their corresponding uniform LBP patterns are different. Here, we denote {{$\bf{LBP^{U}(s, i)}$}} as the uniform LBP pattern on the scale $s$ with $i$ as the start point of the binary sequence, where $0 \le i \le n-1$.

%The image rotation usually changes the LBP value.

To achieve great robustness to image rotation, Ojala et al. also introduced the concept of rotation invariant LBP ({$\bf{LBP^{RI}}$}) and rotation invariant uniform LBP ({$\bf{LBP^{RIU}}$}), where $LBP^{RIU}$ is popularly used for texture classification. The $LBP^{RIU}$ can be defined as:
\begin{equation}
\label{eq:rui}
    LBP^{RIU}(\vec{s}) = \begin{cases}
    \sum_{k=0}^{n-1} \phi(v_k-v_c), &  \Phi(LBP(\vec{s})) \le 2 \\
    n+1, &  otherwise, \\
    \end{cases}
\end{equation}


\begin{multicols}{2}
\begin{figure*}[t]
\begin{center}
 \includegraphics[width=1.0\linewidth]{figures/groupCoLBP.eps}
\end{center}
   \caption{ An illustration of two groups of multi-scale co-occurrence LBPs. Each row denotes one group. In each group, with image rotating, one co-pattern will turn into another one in the same group.}
\label{fig:RotationInvariantCoLBP}
\end{figure*}
\end{multicols}


For the number of neighbors $n=8$, LBP has $2^8=256$ patterns, in which there are 58 uniform patterns and 198 non-uniform patterns. Usually, all 198 non-uniform patterns are regarded as the same pattern. Thus, in practice, $LBP^{U}(8, 1)$ has 59 patterns as shown in Fig. \ref{fig:ulbp}.
According to Eq. \ref{eq:rui}, the $LBP^{RIU}(8, 1)$ has 10 patterns.

%
%\begin{multicols}{2}
%\begin{figure*}[t]
%\begin{center}
% \includegraphics[width=0.85\linewidth]{figures/rulbp.eps}
%\end{center}
%   \caption{A group of LBPs. }
%\label{fig:rlbp}
%\end{figure*}
%\end{multicols}

Multi-scale strategy is widely used in most texture relevant tasks, and it usually boost the classification performance. For instance, the work \cite{ojala2002multiresolution} used three scales ( LBP(8, 1), LBP(16, 2) and LBP(24, 3) ) for texture classification task. To obtain rotation invariance and reduce the feature dimension, $LBP^{RIU}$ is used. Similar with traditional LBP, most LBP variants ( CLBP, LBPHF\_S/M, VLBP, LCP ) also used the multi-scale strategy. The multi-scale strategy has been widely recognized as an indispensable means to achieve superior performance.





\section{Globally Rotation Invariant Multi-scale Co-occurrence LBPs}
\label{sec:RIA}
In this section, we firstly analyze the correlation existing in multiple scales. The strong correlation among the scales motivates the joint encoding of multi-scale co-occurrence. Then,  we introduce the multi-scale co-occurrence of uniform LBP. And then, we detailly introduce and analyze three effective rotation invariant encoding methods. After, we analyze its relationship with single scale LBP. Finally, we introduce the classifier used in this paper.

\subsection{Correlation Analysis between Different Scales}
\label{sec:CADS}
As indicated before, each LBP pattern characterizes a local structure, but its discriminative power is limited by its small described region. For instance, LBP(8, 1) depicts a $3\times 3$ regions.
Though the multi-scale strategy can be used to depict multi-scale information, the traditional multi-scale methods ignore the correlation between different scales.

However there exists strong correlations between different scales. Ignoring the correlation will lead to huge information loss. As shown in Fig. \ref{fig:lbp_and_mslbp}, being effectively encoded, the patterns in multiple scales jointly reflect strong local structures. Below, we will firstly investigate the correlation between different scales.

The LBP patterns in different scales not only contains relevant information, but also has strong complementary information. In the literature
\cite{ojala2002multiresolution, maenpaa2003multi}, the classical multi-scale LBPs proves to significantly outperform the single-scale LBP. This observation shows that the LBPs in multi-scale are complementary. In \cite{qibmvc2}, Qi et al. use information theory to demonstrate the high correlation between different channels. Here, we also use the same tool to analyze the correlation between the LBP patterns in different scales. Table \ref{table:statistics} shows some statistics using  Outex\_00012 dataset \cite{ojala2002outex}.


%
%\begin{figure}[t]
%\begin{center}
% \includegraphics[width=1.0\linewidth]{figures/groupCoLBP.eps}
%\end{center}
%   \caption{An illustration of a group of multi-scale co-occurrence LBPs.}
%\label{fig:RotationInvariantCoLBP}
%\end{figure}




\begin{table}[h]
\caption{Texture Correlation between LBP(8, 1), LBP(8, 2), and LBP(8, 3).}              % title of Table
\centering                                     % used for centering table
%\small
\begin{tabular}{| @{\ }c@{\ } | @{\ }c@{\ } | @{\ }c@{\ } | @{\ }c@{\ } | @{\ }c@{\ } |}                       % centered columns (4 columns)
\hline
((8, 1), (8, 2))                 & H((8, 1))      & H((8, 2))      & H((8, 1), (8, 2))       & I((8, 1), (8, 2))       \\
\hline
Information Entropy    & 4.37      & 4.35      & 6.87          & \bf{1.84}          \\
\hline
((8, 1), (8, 3))                 & H((8, 1))      & H((8, 3))      & H((8, 1), (8, 3))       & I((8, 1), (8, 3))       \\
\hline
Information Entropy    & 4.37      & 4.37      & 7.82          & 0.91          \\
\hline
((8, 2), (8, 3))                 & H((8, 2))      & H((8, 3))      & H((8, 2), (8, 3))       & I((8, 2), (8, 3))       \\
\hline
Information Entropy    & 4.35      & 4.37      & 8.05          & 0.67          \\
\hline

\end{tabular}
\label{table:statistics}                   % is used to refer this table in the text
\end{table}

From Table \ref{table:statistics}, we have the following two key observations: (1): the LBP patterns in different scale have strong correlation. The mutual information is an effective indicator of the correlation. The correlation between LBP(8, 1) and LBP(8, 2) is higher.  (2): With the increase of the distance, the correlation decreases. For example, the correlation between LBP(8, 1) and LBP(8, 2) is greatly higher than that between LBP(8, 1) and LBP(8, 3).





Compared with single LBP, the joint encoding of multi-scale LBPs has two obvious advantages. Firstly, multi-scale LBPs depicts larger regions, thus they can capture stronger structures. 
Secondly, the joint encoding of multi-scale LBPs can capture richer patterns. For instance, for LBP(8, 1), it has 256 patterns. But for the co-occurrence of LBP(8, 1) and LBP(8, 2), it has 65536 co-patterns. Thus, if well encoded, the multi-scale co-occurrence of LBPs will have strong discriminative power.
%As shown in Fig. \ref{fig:lbp_and_mslbp}, the LBPs in multi-scales captures stronger curvature variation.




%\section{Rotation Invariance for Multi-scale Co-occurrence LBPs}
%\label{sec:MCLBP}
%\subsection{LBP and Multi-scale Co-occurrence LBPs}


\subsection{Multi-scale Co-occurrence LBP (MCLBP)}

%Then, we will present the MCLBP in detail.






In natural image, 58 uniform LBP patterns account for most of all 256 patterns. It is observed that the ratio is about 80\% to 90\%. Thus, instead of the original LBP, the uniform LBP is widely used. In this work, we also use uniform LBP though our method can be directly applied to the original LBP.

First, the LBP and ULBP value for each point in required scale was calculated. Then, the multi-scale co-occurrence of  $LBP^U$ (MCLBP) can be denoted as follows:
\begin{equation}
\label{eq:msjLBP}
CoLBP^{UU}(\vec{s_1}, \vec{s_2}) = [LBP^{U}(\vec{s_1}, i), LBP^{U}(\vec{s_2}, i)]_{co},
\end{equation}
where $i$ can be fixed to be any one in $[0, n-1]$. Here, we just set it to 0.

Thus, for each point, its MCLBP pattern can be denoted as a pattern in $59\times 59$. Any image can be denoted into a histogram distribution of these 3481 patterns. Note that This co-occurrence pattern is not rotation invariant. Image rotation will greatly change the histogram distribution.



%To achieve rotation invariance, our task is to extract the rotation invariant feature from the histogram distribution.
There exist some interesting rules among some co-patterns. As shown in Fig. \ref{fig:RotationInvariantCoLBP}, for the patterns in each row, with the image rotating, the patterns will turn into another one in the same row. In this paper, we call all patterns of each row as ``Group''.

According to the defined rule of groups, we can divide all 3841 co-patterns into 433 groups.

% Similar with the single scale LBP, the co-occurrence LBP patterns can be divided into some patterns. The co-occurrence patterns own the same property with single LBP pattern when the images rotate. As shown in \ref{fig:RotationInvariantCoLBP}, the shown eight patterns can be divided into a group. When all co-occurrence patterns are grouped, the same encoding methods in Sec. \ref{sec:RIA} can be applied.
%
%{\bf{Problem Formulation:\ }}In most current applications, LBP is usually divided into the uniform and non-uniform patterns. For the uniform patterns, we can further divide the patterns into different groups according to their properties. Here, we define a concept called ``Group'' for the uniform patterns. We define the $i$th group $G_i$ as:
%\begin{equation}
%\label{eq:set}
%    G: \{G_i \ |\ LBP^{RIU}(\vec{s}) = i \}
%\end{equation}
%%G: \{G(\vec{s},\ i)\ |\ i \in [0, n] \ \}
%where $\vec{s} = [n, r]$. Here, the $i$ can be considered as the number of ``1'' in the binary sequence.


\subsection{Globally Rotation Invariant Encoding Strategy}

%Properties of the uniform groups: (1) with the image rotation, one pattern will change to another pattern which belongs to the same group as the refer pattern.

For an image, its histogram distribution $H$ of all LBP patterns can be calculated. To make the integral probability to ``1'', we normalize the $H$ using $L_1$ norm.
Let $f$ be a feature extraction function, $G_i$ denotes the $i$th group, $H(G_i)$ denotes the probability distribution of each pattern in the group out of all LBP patterns. The $H(G_i)$ has the same dimension with $G_i$. Here, we use $F_i$ to denote the feature extracted from the distribution $H(G_i)$ using the $f$ feature extraction function. We can define the rotation invariant problem as follows:
\begin{equation}
\label{eq:set}
    f: H(G_i) \rightarrow F_i.
\end{equation}
%
%For an image, its histogram distribution of all LBP patterns can be calculated as $H$. Let $H(G_{ij})$ denote the probability distribution of $j$th pattern in $i$th group out of all LBP patterns.
%In ideal condition, the pattern in one group will not turn into another group under image rotation. Thus, the cumulative probability of one group in all patterns is constant under arbitrary image rotation.

There exists strong law between the probability distribution of the patterns in same group under different image rotation. As shown in Fig. \ref{fig:distribution}, when the image rotates 45 degrees, the probability distribution of one group just circularly shifts one unit. Thus, when we design the feature extraction function, the property of the distribution should be well considered. Actually in practice, the variation raw of the probability distribution in each group under different image rotation will facilitate our feature design.



%To achieve rotation invariance, we should extract the invariant features from each group.



For each group $G_i$, we can extract a feature $F_i$ according to the function $f$. The final feature $F$ can be denotes as follows:
\begin{equation}
\label{eq:set}
    F = [F_0,\ F_1, ......,\ F_n,\ F_{n+1}],
\end{equation}
where $n$ is the number of the neighbors.

\begin{figure}[t]
\begin{center}
 \includegraphics[width=1.0\linewidth, height=0.4\linewidth]{figures/aa.eps}
\end{center}
   \caption{The variation of probability distribution of patterns in one group when image rotates 45 degrees. }
\label{fig:distribution}
\end{figure}

Many methods can be used to encode the histogram distribution. Some may have strong discriminative power, but sensitive to image rotation. Vice verse. A desirable feature extraction function should have great balance between the discriminative power and transformation invariance. In this paper, for this purpose, we propose to use three rotation invariant encoding methods.

{\bf{Sum Pooling.}}
Uniform LBP depends on the defined start point of the binary sequence. Image rotation will vary one uniform pattern $A$ to another uniform pattern $B$, but $A$ and $B$ are in the same group. Thus, for an image, the cumulative probability of all patterns in a group -accounting for the all patterns- will not change. Thus, we can define the following feature extraction function $\vec{{F1_i}}$ for gorup $G_i$ as:
\begin{equation}
\label{eq:f1}
\vec{{F1_i}} = [\sum_{j = 1}^{N_i} h(G_{ij})],
\end{equation}
where $N_i$ is the numbers of patterns in group $G_i$.

{\bf{Remark:}} Sum pooling is an effective way to capture the cumulative probability in a group. As we have indicated before, regardless of how many degrees the image rotates, the pattern for each point will just change to another pattern in the same group. Thus, the cumulative probability will not vary.
%in ideal condition, when the image rotates a $360*j \div n$ degrees, the binary sequence just circularly rotates. Thus, the probabilities distribution just circularly rotate along with the image rotation. However, the ideal condition
%Like the binary sequence, along with image rotation, the probabilities in a group circularly rotate along with the image rotation. For instance, as shown in Fig. \ref{fig:distribution}, when the image rotates 45 degrees, the probability of $1$th position will turn to the probability in the $2$th position.
%%the relative position of the will change, but the quantity will not change. Thus, there are some

{\bf{Moment Based Pooling.}}
With the image rotating, the probability distributions of all patterns in one group circularly rotate. In such a probability set, there exist some constant properties besides of the cumulative probability.

In this work, we propose a new method to extract the invariant feature from such a group. The function can be defined as:

\begin{equation}
\label{eq:f2}
\vec{F2_i} = [ m, \ {\sigma}_1 \sum_{j=1}^{N_i} ( h(G_{ij}) - \frac{m}{N_i})^{2}],
\end{equation}
where $N_i$ is the numbers of patterns in group $G_i$, $m = \sum_{i = 1}^{N_i} h(G_{ij})$, ${\sigma}_1$  is a parameter.

%
%The second function can be defined as:
%\begin{equation}
%\label{eq:f22}
%\vec{F2_i} = [ m, \ {\sigma}_1 \sum_{j=1}^{N_i} ( h(G_{ij}) - \frac{m}{N_i})^{2}, \ {\sigma}_2 \sum_{j=1}^{N_i} ( h(G_{ij}) - h(G_{i j+1})^{2}],
%\end{equation}
%
%where $N_i$ is the numbers of patterns in group $G_i$. $G_{i N_i+1}$ is equal to $G_1$, ${\sigma}_1$ and ${\sigma}_2$ are two parameters to balance the weights among the three terms.

{\bf{Remark:\ }} The proposed moment based feature extraction method not only captures the cumulative probability in a group, but also reflects the relative variance between each bin and the mean distribution.


{\bf{Fourier Transformation Pooling.}}
In the work \cite{ahonen2009rotation}, Timo et al. firstly proposed to use fourier transformation to achieve a rotation invariant feature from the uniform patterns. Here, we briefly introduce their method. Firstly, we can calculate the Discrete Fourier Transform (DFT) of all patterns' distributions in a group as follows:

\begin{equation}
\label{eq:f3}
HF(k) = \sum_{j=0}^{N_l-1} G_{lj} \exp^{\frac{-i2 \pi jk}{N_l}},\ \ \ \ \  k = 0,.....,N_l-1
\end{equation}
where $N_l$ is the numbers of patterns in group $G_l$.

%
%\begin{figure}
%\begin{center}
% \includegraphics[width=0.80\linewidth]{figures/lbp_and_mslbp.eps}
%\end{center}
%   \caption{An illustration of LBP and Multi-scale LBP. Compared with LBP, LBPs in multiple scales jointly characterize stronger local structures. The LBP patterns in different scales have high correlation. }
%\label{fig:lbp_and_mslbp}
%\end{figure}


After obtaining the DFT of group $G_l$, since it is a complex data, we need to transform it into a real data, thus, we compute its magnitude. The magnitude for $HF(k)$ can be calculated as:
\begin{equation}
\label{eq:f3}
M(k) = \sqrt{HF(k)\overline{HF(k)}}.
\end{equation}


\begin{multicols}{2}
\begin{figure*}[t]
\begin{center}
 \includegraphics[width=0.85\linewidth]{figures/rulbp.eps}
\end{center}
   \caption{A group of single-scale LBPs. }
\label{fig:rlbp}
\end{figure*}
\end{multicols}


Since the last $N_l$-1 terms are sysmatric, the final fourier transformation histogram can be denoted as:
 \begin{equation}
\label{eq:f22}
\vec{F3_l} = [M(0),\  ....,\  M(N_l/2) ].
\end{equation}



{\bf{Remark:}} The DFT is invariant to the circular rotation of the histogram distribution. Thus, in theory, it is invariant to image rotation. However, the natural images are always captured under arbitrary angle. The histogram distribution is circular rotation only when the rotation degree is the times of $360/n$.



The all 3841 co-patterns can be divided into 433 groups. Thus, the dimension of the sum encoding method is 443 dimension for one co-occurrence pair, and the dimension for moment based pooling is 886. According to the DFT encoding strategy, the dimension for DFT based method is 2200.
As CLBP \cite{guo2010completed}, we can also use the center gray level-dividing the image into two parts according to the average gray value. Then, the feature dimension is two times of the original feature. According to \cite{guo2010completed}, the center gray level can provide significant improvement in some datasets.





\subsection{Generalized to Single-scale LBP}
The encoding strategy introduced above can be directly applied to single-scale LBP. As shown in Fig. \ref{fig:rlbp}, we can also construct some groups like above co-occurrence LBPs. For $n = 8$, as shown in Fig. \ref{fig:ulbp},
we can divide the 58 uniform patterns into 9 groups. For the group $G_1$, as shown in Fig. \ref{fig:rlbp}, it contains just one ``1'' in all eight binary bits. In each group, any pattern can rotate to any another pattern in the same group. Thus, in ideal condition, when the image rotates, the uniform pattern of each point will just turn into another pattern in the same group. In practice, we divide all non-uniform patterns into a group which be denoted as $G_{n+1}$.


\subsection{Classification}
To conduct the classification, we use the nearest neighbor (NN) classifier as the compared previous works though the support vector machine (SVM) always shows better performance. ${\chi}^2$ kernel proves to achieve great performance, and is widely used in previous texture classification task. To make the comparison fair, we also use it. The used ${\chi}^2$ kernel similarity between histogram features $X$ and $Y$ can be calculated as follows:
\begin{equation}
\label{eq:kernel}
S(X, Y) = \sum_{i=1}^{N} \frac{2X_iY_i}{X_i+Y_i},
\end{equation}
Where $N$ is the dimension of $X$ and $Y$. The ${\chi}^2$ kernel shows great performance compared with Linear and RBF kernel. It is widely used in texture classification \cite{guo2010completed} \cite{qi2013bmvc1} \cite{zhao2012rotation}. In this paper, to fairly compare with previous works, we will use the NN or SVM according to their used classifier. We use the Vlfeat \cite{vedaldi2010vlfeat} to conduct some fast computation, such similarity computation. For SVM, instead of carefully tuning the parameters, we use the Libsvm \cite{chang2011libsvm} tool with fixed C=100 for all experiments.




\begin{figure}[h]
\begin{center}
 \includegraphics[width=1.0\linewidth]{figures/outex10_curet.eps}
\end{center}
   \caption{Datasets.}
\label{fig:Datasets}
\end{figure}

